CMU's IWSLT 2024 Simultaneous Speech Translation System

This paper describes CMU's submission to the IWSLT 2024 Simultaneous Speech Translation (SST) task for translating English speech to German text in a streaming manner. Our end-to-end speech-to-text (ST) system integrates the WavLM speech encoder, a modality adapter, and the Llama2-7B-Base model as the decoder. We employ a two-stage training approach: initially, we align the representations of speech and text, followed by full fine-tuning. Both stages are trained on MuST-c v2 data with cross-entropy loss. We adapt our offline ST model for SST using a simple fixed hold-n policy. Experiments show that our model obtains an offline BLEU score of 31.1 and a BLEU score of 29.5 under 2 seconds latency on the MuST-C-v2 tst-COMMON.

==> tables/ablation.tex <==
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \textbf{Stage1} & \textbf{Stage2} & \textbf{Stage1 BLEU} & \textbf{Stage2 BLEU} \\
% \midrule
% Wav2vec + llama2 & $\checkmark$ & $\checkmark$ & - & 30.02 \\
% Wav2vec + Tower & $\checkmark$ & $\checkmark$ & 29.35 & 30.53 \\
% Wavlm + Tower & $\checkmark$ & $\checkmark$ & 30.11 & 31.64 \\
% Wavlm + TowerInstruct & $\checkmark$ & $\times$ & 29.64 & - \\
% Wavlm + Llama & $\checkmark$ & $\checkmark$ & 25.50 & 30.31 \\
% \bottomrule
% \end{tabular}%
% }

\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccc}
\toprule
& \multicolumn{2}{c}{\textbf{Speech Encoder}} \\
\cmidrule(lr){2-5}
\textbf{LLM} & \multicolumn{2}{c}{Wav2vec} & \multicolumn{2}{c}{WavLM} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& stage1  & stage2  & stage1  & stage2  \\
\midrule
TowerInstruct      & - & - & 29.64 & - \\
Tower     & 29.35  & 30.53 & 30.11 & 31.64 \\
LLaMA2     & -  & 30.02 & 25.50 & 30.31 \\
\bottomrule
\end{tabular}%
}


